Asynchronous Parallel Bayesian Optimisation via Thompson Sampling

We design and analyse variations of the classical Thompson sampling (TS) procedure for Bayesian optimisation (BO) in settings where function evaluations are expensive, but can be performed in parallel. Our theoretical analysis shows that a direct application of the sequential Thompson sampling algorithm in either synchronous or asynchronous parallel settings yields a surprisingly powerful result: making $n$ evaluations distributed among $M$ workers is essentially equivalent to performing $n$ evaluations in sequence. Further, by modeling the time taken to complete a function evaluation, we show that, under a time constraint, asynchronously parallel TS achieves asymptotically lower regret than both the synchronous and sequential versions. These results are complemented by an experimental analysis, showing that asynchronous TS outperforms a suite of existing parallel BO algorithms in simulations and in a hyper-parameter tuning application in convolutional neural networks. In addition to these, the proposed procedure is conceptually and computationally much simpler than existing work for parallel BO.

==> _ <==

\section{Introduction}
\label{sec:intro}

In stochastic bandit optimisation, we are tasked with optimising a noisy,
black-box function $\func$.
In typical applications, such as hyper-parameter tuning, experiment design, online
advertising, clinical trials, and scientific experiments, an evaluation of $\func$ incurs
a large economic or computational cost and we need to keep the number of
evaluations to a minimum.
Bayesian optimisation (BO) refers to a suite of methods for bandit optimisation in the
Bayesian paradigm,
which has been successfully used in many of the above applications%
~\citep{snoek12practicalBO,hutter2011smac,martinez07robotplanning,%
parkinson06wmap3,gonzalez14gene}.

That said, most bandit methods are inherently sequential in nature.
That is, an algorithm has to wait for an evaluation to complete
before proceeding to the next.
However, in many applications we may have the opportunity to conduct several evaluations
in parallel.
For instance, in hyper-parameter tuning, today we have computational infrastructure
to train several models in parallel.
In online advertising we might wish to display several ads
to different audiences at the same time.
As a result, there has been a surge of interest in parallelising bandit methods,
particularly in the BO literature.
We contribute to this line of work by studying Thompson Sampling (\ts)%
~\citep{thompson33sampling} for parallelising BO.
By  a direct application of the sequential \tss procedure to the $M$ synchronous or
asynchronously parallel workers, we derive algorithms \syntss and \asyts.
Our \textbf{main contributions} in this work are,
\begin{enumerate}[leftmargin=0.22in]
\item A theoretical analysis of the regret for parallel \ts, demonstrating
that both \syntss and \asytss making $n$ evaluations with $M$ parallel workers 
is almost as good as if the $n$ evaluations were made in sequence.
% as sequential \emph{TS} with $M$ times as many evaluations.
\insertitemspacing
\item An analysis 
\insertitemspacing
\item An empirical evaluation whic demonstrates that \asytss significantly outperforms
existing methods for parallel BO.
\end{enumerate}

\subsection*{Related Work}

To cite:~\citep{ginsbourger2011dealing,janusevskis2012ei,wang2016parallel,%
gonzalez2015batch,desautels2014parallelizing,contal2013parallel,shah2015parallel,%
kathuria2016bodpps,wang2017batched}.
A few more to add.

When compared to existing work on parallel Bayesian optimisation, our approach has one
or more of the following advantages.
\begin{enumerate}[leftmargin=0.2in]
\item \textbf{Asynchronicity:}
The majority of work on parallel BO are in the synchronous (batch) setting.
To our knowledge, only~\citep{ginsbourger2011dealing,janusevskis2012ei,wang2016parallel}
focus on asynchronous parallelisation.
\insertitemspacing
\item \textbf{Theoretical underpinnings:}
% Besides some work work using upper confidence bound techniques~\citep{kathuria2016bodpps,%
% contal2013parallel,desautels2014parallelizing}, the rest of the methods do not come
% with theoretical guarantees.
Most methods for parallel BO do not come with theoretical guarantees (with the exception
of some work using UCB techniques~\citep{kathuria2016bodpps,%
contal2013parallel,desautels2014parallelizing}).
Crucially, to the best of our knowledge, this includes all work in the asynchronous
setting.
\insertitemspacing
\item \textbf{Computationally and conceptually simple:}
When extending a sequential BO algorithm to the parallel setting, most methods either
introduce additional hyper-parameters~\citep{gonzalez2015batch},
ancillary computational routines~\citep{kathuria2016bodpps,desautels2014parallelizing},
or require optimising an $Md$ dimensional acquisition~\citep{wang2016parallel}.
In contrast, our approach is conceptually simple -- a direct application of the
sequential TS algorithm to the parallel workers.
It does not introduce any additional hyper-parameters or ancillary routines and
computationally is only as difficult as sequential BO methods.
\end{enumerate}

It should be emphasised that using parallelised \tss is not entirely novel
and has been explored to varying degrees in applied domains of bandit and re-inforcement
learning research~\citep{osband2015bootstrapped,israelsen2017towards,%
hernandez2016distributed,osband2016deep}.
However, to our knowledge, we are the first to theoretically analyse parallel \ts.
More importantly, we are also the first to propose and analyse \tss in an asynchronous
parallel setting.



==> implementation.tex <==

\begin{comment}
\subsection{Implementation}
\label{sec:implementation}
\vspace{-0.05in}

While the analysis assumes that the GP prior is known, this is hardly the case in
practice.
In our experiments, following recommendations
in~\citep{snoek12practicalBO,kandasamy15addBO},
the implementation of \synts, \asyts, and other BO techniques
estimates the kernel using its past evaluations and updates it every $25$ iterations.
Next, consider initialisation.
The initialisation scheme in Proposition~\ref{prop:initialisation}
is not always practical as it will require that we know the kernel $\kernel$ of the GP at
the beginning of the optimisation routine.
In our experiments, we replace this by initialising TS (and other BO methods) with
some evaluations at randomly selected points.
Mismatch between theory and practice is not uncommon in BO. 
For example, most papers, including ours, assume that the prior kernel $\kernel$ is known in 
theory.
In practice however, $\kernel$ is typically estimated on the fly as described above.
However, the initialisation scheme requires that we know the kernel \emph{before}
collecting any data which is problematic.
Random initialisation on the other hand, is more standard in the BO
literature~\citep{snoek12practicalBO}
and at least partially achieves the effect of minimising the variance throughout the
domain.
% \toworkon{I don't like how this para reads.}

% \akshay{I don't like calling them discouraging, it sounds very negative. What about something like ``explicit diversity." Or ``deliberate."}
\end{comment}


==> zz_ancillary.tex <==

\section{Some Ancillary Material}
\label{app:ancillary}

\subsection{Some Results on GPs and GP bandits}
\label{app:gps}

We will provide our bounds in terms of the \emph{Maximum Information Gain} (\mig)
which characterises the statistical difficulty of GP bandits.

\insertthmprespacing
\begin{definition}[Maximum Information Gain~\citep{srinivas10gpbandits}]
Let $f\sim \GP(\zero, \kernel)$
where $\kernel:\Xcal^2\rightarrow \RR$.
Let $A = \{x_1, \dots, x_n\} \subset \Xcal$ be a finite subset.
Let $f_{A}, \epsilon_{A}\in\RR^n$ such that $(f_{A})_i=f(x_i)$ and
$(\epsilon_{A})_i\sim\Ncal(0,\eta^2)$.
Let $y_{A} = f_{A}+\epsilon_{A} \in \RR^n$.
Denote the Shannon Mutual Information by $I$.
The Maximum Information Gain is
\[
\IGn = \max_{A\subset \Xcal, |A| = n} I(y_{A}; f_{A}).
\]
\label{def:infGain}
\end{definition}
% \insertthmpostspacing

% The \migs was introduced by~\citep{srinivas10gpbandits} who also 
\citet{srinivas10gpbandits} and~\citet{seeger08information} provide
bounds on the \migs for different classes of kernels.
For example for the SE kernel, $\IGn\asymp \logn^{d+1}$
and for the \matern kernel with parameter $\nu$,
$\IGn \asymp n^{\frac{d(d+1)}{2\nu + d(d+1)}}\logn$.
The next theorem due to~\citet{srinivas10gpbandits} bounds the sum of variances
of a GP using the~\mig.

\toworkon{Double Check this!!}
\akshay{The original proof uses that $x_t$ is deterministic conditioned in $y_{1:t-1}$. This is not true in our case.
  I guess for us the analog of Lemma 5.3 in Srinivas et al. is}
  \begin{align*}
    \akshay{I(y_{1:n};f) \ge \sum_{j=1}^n \EE_{x_j} \frac{1}{2}\log(1 + \eta^{-2}\sigma_{j-1}(x_j)).}
  \end{align*}
\akshay{For this I had to use Jensen's inequality and concavity of
  entropy since $y_j |y_{1:j-1}$ is drawn from a mixture of Gaussians,
  since $x_j$ is random. I don't see another way to overcome the
  random choice of $x_j$. Honestly I think Srinivas et al. also need
  the expectation there, but they can preserve equality.}

For synchronous parallel, using the above inequality and notice that in the same batch, the distribution over $x_j$ and posterior variance are fixed, we instead get
\begin{align*}
I(y_{1:n};f) \ge M\sum_{j=1}^{n/M} \EE_{x \sim P_j} \frac{1}{2}\log(1+\eta^{-2}\sigma_{j}(x_j))
\end{align*}
\akshay{Samy you will have to fix the indexing}

\insertthmprespacing
\begin{lemma}
\label{lem:IGBoundLemma}
Let $\func\sim\GP(0,\kernel)$, $\func:\Xcal\rightarrow\RR$ and each time we query at
any $x\in\Xcal$ we observe $y = \func(x)+\epsilon$, where
$\epsilon\sim\Ncal(0,\eta^2)$.
Let $A=(\xj)_{t=1}^n$ be any set of $n$ evaluations of $\func$ where $\xj\in\Xcal$ for all
$j$ and $\sigmasqtmo$ denote the posterior variance at time $t$, i.e. after $t-1$ queries.
Then, $\sum_{\xj\in A}\sigmasqtmo(\xj)\leq \frac{2}{\log(1+\eta^{-2})}\IGn$.
% \newcommand{\xAss}[1]{x_{(#1)}}
\end{lemma}
\insertthmpostspacing


Next we will need the following regularity conditions on the derivatives of the
GP sample paths.
When $\func\sim\GP(\zero,\kernel)$, it is satisfied when $\kernel$ is four times
differentiable, e.g. the SE kernel and \matern{} kernel when
$\nu>2$~\citep{ghosal06gpconsistency}.

\insertthmprespacing
\begin{assumption}[Gradients of GP Sample Paths~\citep{ghosal06gpconsistency}]
Let $\func\sim\GP(\zero,\kernel)$, where
$\kernel:\Xcal^2 \rightarrow \RR$ is a stationary kernel.
%  $\kernel(\cdot, x)$ is $L$-Lipschitz for all $x$. 
The partial derivatives
of $\func$  satisfies the following condition.
There exist constants $a, b >0$ such that,
\[
\text{for all $J>0$, $\;$and for all $i \in \{1,\dots,d\}$},\quad \PP\left( \sup_{x} 
\Big|\partialfrac{x_i}{\func(x)}\Big| > J \right)
\leq a e^{-(J/b)^2}.
\]
\label{asm:kernelAssumption}
\end{assumption}
% \insertthmpostspacing

Finally, we will need the following result on the supremum of a Gaussian process.
It is satisfied when $\kernel$ is twice differentiable.

\insertthmprespacing
\begin{fact}[Supremum of a GP~\citep{adler1990gps}]
\label{fact:supgp}
Let $\func\sim\GP(0,\kernel)$ have continuous sample paths.
Then, $\EE\|\func\|_\infty = \supgp < \infty$.
\end{fact}
This, in particular implies that in the definition of $\bsrtT$ in~\eqref{eqn:srtDefn},
$\max_{x\in\Xcal}|f(\xopt) - f(x)| \leq 2\supgp$.

\subsection{Some Results on Concentration of Measure}
\label{app:concmeasure}

\subsection{Other bounds on the MIG}
\akshay{Here are some thoughts on a synchronous bound. I think you
  lose essentially nothing except for if a particular matrix can be
  singular. Let's see the lower bound.
}

\begin{align*}
I(y_n;f) &= H(y_n) - \frac{n}{2}\log(2\pi e \eta^2) = \sum_{B=1}^{n/M} H(y_B | y_{1:B-1}) - \frac{n}{2}\log(2\pi e \eta^2)\\
&\ge \sum_{B=1}^{n/M} \EE_{x_1^M\sim P_B} \frac{1}{2}\log(2\pi e |\eta^2 I + K_B(x_1^M)|) - \frac{n}{2}\log(2\pi e \eta^2)\\
& = \sum_{B=1}^{n/M} \EE_{x_1^M\sim P_B} \frac{1}{2}\log(|I + \eta^{-2}K_B(x_1^M)|)
\end{align*}
Here $B$ is used to denote a batch and $y_B$ consists of $M$ samples.
The inequality uses Jensen's inequality and concavity to pull the
expectation over $x_1^M$ out of the entropy.  Then we use the fact
that $y_B | x_1^M \sim \Ncal(\cdot, K_B(x_1^M) + \eta^2 I)$ where
$K_B$ is the posterior kernel after $B-1$ batches. $P_B$ is the TS
sampling distribution.

Now we use the inequality
\begin{align*}
\log \det A \ge \tr( I - A^{-1}),
\end{align*}
which is just $1-1/x \le \log x$ in disguise. We also use the
Sherman-Morrison-Woodbury identity, which states that
\begin{align*}
(I + XX^T)^{-1} = I - X(I + X^TX)^{-1}X^T.
\end{align*}
By the fact that $K_B(x_1^M)$ is positive semidefinite, we can write $\eta^{-2}K_B(x_1^M) = VV^T$ and obtain
\begin{align*}
\log(|I + \eta^{-2}K_B(x_1^M)|) &\ge \tr(I - (I+VV^T)^{-1})\\
& = \tr(V(I+V^TV)^{-1}V^T)
 = \tr((I+V^TV)^{-1}V^TV).
\end{align*}
This last expression is a product of two matrices that are
simultaneously diagonalizable. One has eigenvalues $\lambda_j$ and the
other has $(1+\lambda_j)^{-1}$. We don't know what the eigenvalues
are, but we do know that $\sum_j\lambda_j = \tr(V^TV) = \tr(VV^T) =
\sum_{j=1}^M\eta^{-2}\sigma_B^2(x_j)$, which is essentially what we
want. Note that we don't even know the rank.

We can get an easy lower bound
\begin{align*}
I(y_n;f) &\ge \sum_{B=1}^{n/M}\frac{1}{2}\EE_{x_1^M\sim P_B} \sum_{j=1}^M \frac{\eta^{-2} \sigma_B^2(x_j)}{1+\lambda_{\max}(\eta^{-2}K_B(x_1^M))}
\ge \sum_{B=1}^{n/M}\frac{1}{2}\EE_{x_1^M\sim P_B} \sum_{j=1}^M \frac{\eta^{-2} \sigma_B^2(x_j)}{1+\sum_{j=1}^M\eta^{-2}\sigma_B^2(x_j)}\\
& \ge \sum_{B=1}^{n/M}\frac{1}{2}\frac{M\eta^{-2}}{1+M\eta^{-2}} \EE_{x\sim P_B}\sigma_B^{2}(x)
\end{align*}
This is adequate to control the synchronous regret but you lose a
multiplicative $M$ factor. However this only happens in the rank-1
case, which happens with probability zero under the TS sampling.
Instead we want to exploit that $K_B(x_1^M)$ should be well
conditioned, which seems plausible if we are playing stochastically,
but I am stuck here for now.

We need to bound the largest eigenvalue of the kernel matrix
$K_B(x_1^M)$. We get a matrix concentration result essentially for
free:
\begin{align*}
\PP\left(\left|\lambda_{\max}(K_B(x_1^M)) - \EE \lambda_{\max}(K_B(x_1^M))\right| \ge M\epsilon \right) \le 2\exp\left(-2\epsilon^2M/R^4\right).
\end{align*}
See Shaw-Taylor's paper. So now we need to bound the expected largest eigenvalue. 

